What a Comfortable World: Ergonomic Principles Guided Apartment Layout Generation

Current data-driven floor plan generation methods often reproduce the ergonomic inefficiencies found in real-world training datasets. To address this, we propose a novel approach that integrates architectural design principles directly into a transformer-based generative process. We formulate differentiable loss functions based on established architectural standards from literature to optimize room adjacency and proximity. By guiding the model with these ergonomic priors during training, our method produces layouts with significantly improved livability metrics. Comparative evaluations show that our approach outperforms baselines in ergonomic compliance while maintaining high structural validity.

==> floor_plans_samples_table.tex <==
\begin{figure*}[t]
\centering

\begin{minipage}{0.31\textwidth}
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{@{}c@{}c@{}c@{}}
        \textbf{Our} & \textbf{Baseline} & \textbf{RPLAN} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_0.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_0.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_0.svg} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_1.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_1.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_1.svg} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_2.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_2.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_2.svg} \\

        
    \end{tabular}
\end{minipage}
\hfill
\begin{minipage}{0.31\textwidth}
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{@{}c@{}c@{}c@{}}
        \textbf{Our} & \textbf{Baseline} & \textbf{RPLAN} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_4.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_4.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_4.svg} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_5.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_5.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_5.svg} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_6.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_6.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_6.svg} \\

        
    \end{tabular}
\end{minipage}
\hfill
\begin{minipage}{0.31\textwidth}
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{@{}c@{}c@{}c@{}}
        \textbf{Our} & \textbf{Baseline} & \textbf{RPLAN} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_8.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_8.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_8.svg} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_9.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_9.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_9.svg} \\

        \includesvg[width=0.33\linewidth]{imgs/our/our_10.svg} &
        \includesvg[width=0.33\linewidth]{imgs/baseline/baseline_10.svg} &
        \includesvg[width=0.33\linewidth]{imgs/gt/gt_10.svg} \\
        
        
    \end{tabular}
\end{minipage}
\caption{Qualitative comparison of results between baseline, our method and samples form RPLAN dataset.}
\ref{fig:qualitative_comparison}

\end{figure*}

